Improved entanglement indicators for optical fields and its application in the event-ready experiment for bright squeezed vacuum with induced non-gaussianity

Better versions of separability conditions for four mode optical fields, i.e. two beams with two modes of mutually orthogonal polarization are given. Our conditions involve variances. Their meaning is intuitive and their implementation is feasible. Namely, if for a given quantum state the spread of the data around its mean value is smaller than the minimal spread predicted for the set of separable states, then the given state is entangled. Our conditions are formulated for standard quantum Stokes observables and normalized Stokes observables and result to be more efficient that the previous conditions for four mode optical fields involving variances. We test our conditions for bright squeezed vacuum with (and without) induced non-gaussianity obtained by addition or subtraction of photons. Also we propose a practical experimental scheme of how to generate such states for an event-ready experiment.

==> notes.tex <==
Condition (\ref{VARNEW}) is suitable for detection of entanglement of states that exhibit anticorrelations such as $\ket{\Psi^-}$. However, we can consider other macroscopic analogs of three others maximally entangled two-qubit states that together with  EPR singlet $\ket{\psi^-}$ form Bell basis. We have '' macroskopic Bell states basis" \cite{GENERAL}:
\begin{equation}
\ket{\Phi^{\pm}} =
\frac{1}{\cosh^2(\Gamma)}\sum_{n=0}^\infty \frac{\tanh^n(\Gamma)}{n!} (a_H^\dagger b_H^{\dagger}\pm a_V^\dagger b_V^{\dagger})^n \ket{\Omega},
\label{\phi}
\end{equation}
and
\begin{equation}
\ket{\Psi^{\pm}} =
\frac{1}{\cosh^2(\Gamma)}\sum_{n=0}^\infty \frac{\tanh^n(\Gamma)}{n!} (a_H^\dagger b_V^{\dagger}+ a_V^\dagger b_H^{\dagger})^n \ket{\Omega}.
\label{psi}
\end{equation}

Obviously condition (\ref{VAR1new}) is not optimal for $\ket{\Psi^+}$ and $\ket{\Phi^{\pm}}$. Hence we present entanglement condition based on variance in arbitrary direction. 

